Faithful Edge Federated Learning: Scalability and Privacy

Federated learning enables machine learning algorithms to be trained over a network of multiple decentralized edge devices without requiring the exchange of local datasets. Successfully deploying federated learning requires ensuring that agents (e.g., mobile devices) faithfully execute the intended algorithm, which has been largely overlooked in the literature. In this study, we first use risk bounds to analyze how the key feature of federated learning, unbalanced and non-i.i.d. data, affects agents' incentives to voluntarily participate and obediently follow traditional federated learning algorithms. To be more specific, our analysis reveals that agents with less typical data distributions and relatively more samples are more likely to opt out of or tamper with federated learning algorithms. To this end, we formulate the first faithful implementation problem of federated learning and design two faithful federated learning mechanisms which satisfy economic properties, scalability, and privacy. Further, the time complexity of computing all agents' payments in the number of agents is $\mathcal{O}(1)$. First, we design a Faithful Federated Learning (FFL) mechanism which approximates the Vickrey-Clarke-Groves (VCG) payments via an incremental computation. We show that it achieves (probably approximate) optimality, faithful implementation, voluntary participation, and some other economic properties (such as budget balance). Second, by partitioning agents into several subsets, we present a scalable VCG mechanism approximation. We further design a scalable and Differentially Private FFL (DP-FFL) mechanism, the first differentially private faithful mechanism, that maintains the economic properties. Our mechanism enables one to make three-way performance tradeoffs among privacy, the iterations needed, and payment accuracy loss.

==> Sec-reference.tex <==
%!TEX root = Main-DASH-AUCTION.tex
%SourceDoc Main-DASH-AUCTION.tex


\begin{thebibliography}{99}

\bibitem{spetrum}
G. Ding, J. Wang, Q. Wu, L. Zhang, Y. Zou, Y. D. Yao, and Y. Chen, ``Robust spectrum sensing with crowd sensors,'' \textit{IEEE Tran. Commun.},  2014.



\bibitem{wefi}
``WeFi'', \url{www.wefi.com/}.

\bibitem{Open}
``OpenSignal,'' \url{http://opensignal.com/}.

\bibitem{waze}
``Waze'', \url{www.waze.com/}.

\bibitem{smartparking}
B. Hoh, T. Yan, D. Ganesan, K. Tracton, T. Iwuchukwu and J. Lee, ``TruCentive: A game-theoretic incentive platform for trustworthy mobile crowdsourcing parking services,''  \textit{IEEE  ITSC}, 2012.

\bibitem{MC10}
X. Zhang \textit{et al.}, ``Incentives for Mobile Crowd Sensing: A Survey,'' \textit{IEEE Communications Surveys Tutorials}, 2016.

\bibitem{Waze1}
K. D. Atherton, ``Israeli Students Spoof Waze App With Fake Traffic Jam". \textit{Popular Science,} 2015.

\bibitem{Waze2}
S. Hendrix, ``Traffic-weary homeowners and Waze are at war, again. Guess who's winning?'' \textit{The Washington Post}, 2016.

\bibitem{Maksin1}
E. Maskin, ``Auction and privatization.'' in Privatization, ed. by H. Siebert. Kiel: Institutfuer Weltwirtschaft der Universtaet Kiel, 115-136, 1992.

\bibitem{Maksin2}
P. Dasgupta and E. Maskin, ``Efficient auctions,'' \textit{Quarterly Journal of Economics}.

%
%\bibitem{Superm}
%D. M. Topkis, ``Minimizing a submodular function on a lattice.'' \textit{Operations research}, 26(2), pp.305-321, 1978.



\bibitem{interdependentval}
P. Jehiel and B. Moldovanu, ``Efficient design with interdependent valuations.'' \textit{Econometrica},  2001.

\bibitem{Interdependence}
C. Mezzetti, ``Mechanism design with interdependent valuations: Efficiency.'' \textit{Econometrica},  2004.

\bibitem{interde}
R. P. McLean and A. Postlewaite, ``Implementation with interdependent valuations.'' \textit{Theoretical Economics}, 2016.





\bibitem{MCS1}
I. Koutsopoulos, ``Optimal incentive-driven design of participatory sensing systems,''
in \textit{Proc. IEEE INFOCOM},
2013.

\bibitem{MCS2}
N. B. Shah and D. Zhou, ``Double or nothing: Multiplicative incentive mechanisms
for crowdsourcing,'' in \textit{Proc. NIPS},
2015.

\bibitem{MCS3}
L. Duan, T. Kubo, K. Sugiyama, J. Huang, T. Hasegawa, and J. Walrand, ``Incentive
mechanisms for smartphone collaboration in data acquisition and distributed
computing,'' in \textit{Proc. IEEE INFOCOM},
2012.

\bibitem{MCS4}
D. Yang, G. Xue, X. Fang, and J. Tang, ``Crowdsourcing to smartphones: Incentive
mechanism design for mobile phone sensing,'' in \textit{Proc. ACM MobiCom}, 2012.

% \bibitem{MCS44}
% X. Zhang, G. Xue, R. Yu, D. Yang and J. Tang, ``Truthful incentive mechanisms for crowdsourcing,'' in \textit{Proc. IEEE INFOCOM},  2015.


% \bibitem{MCS5}
% Z. Feng, Y. Zhu, Q. Zhang, L. M. Ni, and A. V. Vasilakos, ``Trac: Truthful auction
% for location-aware collaborative sensing in mobile crowdsourcing,'' in \textit{Proc. IEEE
% 	INFOCOM}, 2014.



\bibitem{MCS7}
W. Wang, L. Ying, and J. Zhang, ``The value of privacy: Strategic data subjects,
incentive mechanisms and fundamental limits,'' in \textit{Proc. ACM SIGMETRICS}, 2016.

\bibitem{MCS10}
Y. Chen, X. Wang, B. Li, and Q. Zhang, 2019, ``An incentive mechanism for crowdsourcing systems with network effects.'' \textit{ACM TOIT}, 2019.





%\bibitem{MCS10}
%H. Jin, L. Su, and K. Nahrstedt, ``Theseus: Incentivizing Truth Discovery in Mobile Crowd Sensing System,'' in \textit{Proc. ACM MobiHoc}, 2017.

\bibitem{MCS6}
Y. Luo, N. B. Shah, J. Huang, and J. Walrand, ``Parametric prediction from parametric
agents,'' \textit{Oper. Res.}, 2018.

\bibitem{MCS11}
D. Peng, F. Wu and G. Chen, ``Data quality guided incentive mechanism design for crowdsensing,'' \textit{IEEE TMC}, 2018.




\bibitem{MCS12}
H. Jin, L. Su, and K. Nahrstedt, ``Theseus: Incentivizing truth discovery in mobile
crowd sensing systems,'' in \textit{Proc. ACM MobiHoc}, 2017.


\bibitem{MCS8}
X. Gong and N. B. Shroff, "Truthful mobile crowdsensing for strategic users with private data quality," \textit{IEEE/ACM ToN},  2019.

\bibitem{MCS9}
X. Gong and N. Shroff, ``Incentivizing truthful data quality for quality-aware mobile data crowdsourcing.'' in \textit{Proc. ACM Mobihoc}, 2018.

%\bibitem{MCS11}
%L. Pu, X. Chen, J. Xu and X. Fu, ``Crowdlet: Optimal worker recruitment for self-organized mobile crowdsourcing,'' in \textit{IEEE INFOCOM}, 2016.





%\bibitem{Superm}
%D. M. Topkis, ``Minimizing a submodular function on a lattice.'' \textit{Operations research}, 26(2), pp.305-321, 1978.





\bibitem{Vickery}
W. Vickery, ``Counterspeculation, auctions and competitive sealed tenders,''
\textit{Journal of Finance}, 1961.

\bibitem{Clarke}
E. Clarke, ``Multipart pricing of public goods,''
\textit{Public Choice}, vol. 11,
no.1, pp. 17-33, 1971.

\bibitem{Groves}
T. Groves, ``Incentives in Teams,''
\textit{Econometrica}, 1973.

\bibitem{VCG}
S. Yang, and B. Hajek,  ``VCG-Kelly mechanisms for allocation of divisible goods: Adapting VCG mechanisms to one-dimensional signals,'' \textit{IEEE J. Sel. Areas Commun.}, 2007.

\bibitem{surrogate}
R. Johari and J.N. Tsitsiklis,   ``Efficiency of scalar-parameterized mechanisms,'' \textit{Oper. Res.},  2009.


% \bibitem{MD3}
% H. Ge and R. A. Berry, ``Dominant strategy allocation of divisible
% network resources with limited information exchange'', in \textit{Proc. IEEE
% 	INFOCOM,} 2018.

\bibitem{MD4}
H. Ge and R. A. Berry, ``Quantized VCG Mechanisms for polymatroid environments'', in \textit{Proc.  ACM MobiHoc,} 2019.

\bibitem{MD1}
A. Kakhbod and D. Teneketzis, ``An efficient game form for multi-rate
multicast service provisioning,'' \textit{IEEE J. Sel. Areas Commun.}, 2012.


\bibitem{MD2}
A. Kakhbod and D. Teneketzis, ``Power allocation and spectrum sharing
in multi-user, multi-channel systems with strategic users,'' \textit{IEEE Trans.
	Autom. Control}, 2012.



\bibitem{NUM}
M. Zhang and J. Huang, ``Efficient network sharing with asymmetric constraint information,'' \textit{IEEE J. Sel. Areas Commun.}, 2019.

\bibitem{WPT}
M. Zhang, J. Huang, and R. Zhang, ``Wireless power transfer with information asymmetry: A public goods perspective,'' \textit{IEEE TMC}, 2019.

\bibitem{auction}
V. Krishna, \textit{Auction theory.} Academic press, 2009.





\bibitem{order}
B. C. Arnold, N. Balakrishnan, and H. N. Nagaraja,  \textit{A first course in order statistics,}  1992.

\bibitem{nonlinear}
 D. P. Bertsekas, \textit{Nonlinear Programming}. Athena Scientific, 2 ed., 1999.


%\bibitem{mini}
%S. Reichelstein and S. Reiter, ``Game forms with minimal message spaces,''
%\textit{Econometrica,} 1988.


%\bibitem{Truth}
%D. Prelec, ``A Bayesian truth serum for subjective data.'' \textit{Science}, 2004.
%
%\bibitem{Truth2}
%T. Gneiting and A. E. Raftery, ``Strictly proper scoring rules, prediction, and estimation.'' \textit{Journal of the American Statistical Association},  2007.


%\bibitem{Scalar}
%R. Johari, J.N. and Tsitsiklis, ``Efficiency of scalar-parameterized mechanisms.'' \textit{Operations Research}, 57(4), pp.823-839, 2009.



%\bibitem{Kelly}
%S. Yang, and B. Hajek, ``VCG-Kelly mechanisms for allocation of divisible goods: Adapting VCG mechanisms to one-dimensional signals.'' \textit{IEEE Journal on Selected Areas in Communications}, 25(6), 2007.



\bibitem{alpha}
J. Mo, and J. Walrand,  ``Fair end-to-end window-based congestion control.'' \textit{IEEE/ACM Trans. Netw.}, 2000.

\bibitem{PBE}
D. Fudenberg and J. Tirole, ``Perfect Bayesian equilibrium and sequential equilibrium.'' \textit{Journal of Economic Theory,} 1991.




\bibitem{Selling}
J. Créemer, and R.P. McLean, ``Optimal selling strategies under uncertainty for a discriminating monopolist when demands are interdependent'', \textit{Econometrica}, 1985.


\bibitem{convex}
S. Boyd and L. Vandenberghe,  \textit{Convex optimization}, Cambridge university press, 2004.
%
%
%\bibitem{technical}
%Technical Report, \url{http://jianwei.ie.cuhk.edu.hk/publication/AppendixNetEcon19Meng.pdf}.

\bibitem{ss}
W. Zhang, R. K. Mallik, and K. B. Letaief, ``Optimization of cooperative spectrum sensing with energy detection in cognitive radio networks.'' \textit{IEEE TWC,}  2009.

% \bibitem{UPN}
% G. Iosifidis, L. Gao, J. Huang, and L. Tassiulas, ``Efficient and fair
% collaborative mobile Internet access,'' \textit{IEEE/ACM Trans. Netw.}, 2017.

% \bibitem{appendix}
% ``Truthful mobile crowdsensing with interdependent valuations'', technical report. \url{http://ncel.ie.cuhk.edu.hk/TRMobiHocMeng}

\end{thebibliography}

